On the geometry of the Humbert surface of square discriminant

For every positive integer $N$ we determine the Enriques--Kodaira type of the Humbert surface of discriminant $N^2$ which parametrises principally polarised abelian surfaces that are $(N,N)$-isogenous to a product of elliptic curves. A key step in the proof is to analyse the fixed point locus of a Fricke-like involution on the Hilbert modular surface of discriminant $N^2$ which was studied by Hermann and by Kani and Schanz. To this end, we construct certain "diagonal" Hirzebruch--Zagier divisors which are fixed by this involution. In our analysis we obtain a genus formula for these divisors, which includes the case of modular curves associated to (any) extended Cartan subgroup of $\mathrm{GL}_2(\mathbb{Z}/N\mathbb{Z})$ and which may be of independent interest.

==> figures/cusp-pics/0mod8_21.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
% N 2 (4)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{tikzpicture}[baseline=(current bounding box.center), yscale=0.8]
  \draw[line width=1.1mm] (-2,0.25) -- (-2,1.75); \node at (-2,1.95)[anchor=east]{$\tilde{F}_{(\weyl,{\weyl})}^+$}; %F_1
  \draw[line width=1.1mm] (2,0.25) -- (2,1.75); \node at (2,1.95)[anchor=west]{$\tilde{F}_{(\weyl,{\weyl})}^+$}; %F_1
  \draw (-3.5,1) -- (3.5,1);
\end{tikzpicture}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../../main"
%%% End:


==> figures/cusp-pics/2mod4_21.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
% N 2 (4)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{tikzpicture}[baseline=(current bounding box.center), yscale=0.8]
  \draw[line width=1.1mm] (-2,0.25) -- (-2,1.75); \node at (-2,1.95)[anchor=east]{$\tilde{F}_{(\weyl,\weyl)}^+$}; %F_1
  \draw[line width=1.1mm] (2,0.25) -- (2,1.75); \node at (2,1.95)[anchor=west]{$\tilde{F}_{(\weyl,\weyl)}^+$}; %F_1
  \draw (-3.5,1) -- (3.5,1);
\end{tikzpicture}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../../main"
%%% End:


==> figures/cusp-pics/4mod8_21.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
% N 2 (4)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{tikzpicture}[baseline=(current bounding box.center), yscale=0.8]
  \draw[line width=1.1mm] (-2,0.25) -- (-2,1.75); \node at (-2,1.95)[anchor=east]{$\tilde{F}_{(\weyl,\weyl)}^+$}; %F_1
  \draw[line width=1.1mm] (2,0.25) -- (2,1.75); \node at (2,1.95)[anchor=west]{$\tilde{F}_{(\weyl,\weyl)}^+$}; %F_1
  \draw (-3.5,1) -- (3.5,1);
\end{tikzpicture}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../../main"
%%% End:

